To Code, or Not To Code? Exploring Impact of Code in Pre-training

Including code in the pre-training data mixture, even for models not specifically designed for code, has become a common practice in LLMs pre-training. While there has been anecdotal consensus among practitioners that code data plays a vital role in general LLMs' performance, there is only limited work analyzing the precise impact of code on non-code tasks. In this work, we systematically investigate the impact of code data on general performance. We ask "what is the impact of code data used in pre-training on a large variety of downstream tasks beyond code generation". We conduct extensive ablations and evaluate across a broad range of natural language reasoning tasks, world knowledge tasks, code benchmarks, and LLM-as-a-judge win-rates for models with sizes ranging from 470M to 2.8B parameters. Across settings, we find a consistent results that code is a critical building block for generalization far beyond coding tasks and improvements to code quality have an outsized impact across all tasks. In particular, compared to text-only pre-training, the addition of code results in up to relative increase of 8.2% in natural language (NL) reasoning, 4.2% in world knowledge, 6.6% improvement in generative win-rates, and a 12x boost in code performance respectively. Our work suggests investments in code quality and preserving code during pre-training have positive impacts.

==> tables/architecture.tex <==
\begin{table}
    \centering
    \resizebox{\textwidth}{!}{
\begin{NiceTabular}{@{}lccccccccc@{}}
\toprule
& Embedding & Num & FFN hidden & Num & Num KV & Head & Vocab & Embedding & Non-embedding\\
& dims & layers & dims & heads & heads & size & size & parameters & parameters\\
\midrule
\aya-23-8B & 4096 & 32 & 22528 & 32 & 8 & 128 & 256000 & 1,048,576,000 & 6,979,457,024\\
\aya-23-35B & 8012 & 40 & 45056 & 64 & 64 & 128 & 256000 & 2,097,152,000 & 32,883,679,232\\
\bottomrule
\end{NiceTabular}
}
\caption{Architecture parameters for \aya 23 model family}
\label{tab:architecture}
\end{table}


==> tables/old-result-table.tex <==
\begin{table*}[t]
    \centering
    \small
    \resizebox{\textwidth}{!}{
\begin{NiceTabular}{l>{\columncolor{gray!20}}l>{\columncolor{gray!20}}lccccccc}[colortbl-like]
\toprule
\multirow{1}{*}{Model Variant}&\multicolumn{2}{c}{Token Count}&\multicolumn{2}{c}{Natural Language}&\multirow{2}{*}{Code}&\multirow{2}{*}{NL Avg.}&\multirow{2}{*}{Total Avg.}\\
\cmidrule(lr){2-3} \cmidrule(lr){4-5}
% \cmidrule(lr){4-5}
&Text&Code&Reasoning&Knowledge\\
\noalign{\smallskip} 
\hline
\noalign{\smallskip} 
\multicolumn{2}{l}{\textsc{\textbf{Pre-training}}} \\
\noalign{\smallskip} 
Code &~~~-&200B&44.7&1.5&15.5&23.1&20.6\\
%Text (200B ckpt.)&200B&~~~-&51.2&9.1&0.2&30.2&20.2\\
Balanced (200B ckpt.) &100B&100B&52.0&7.4&7.8&29.6&22.4\\
Text (400B ckpt.)&400B&~~~-&49.0&9.5&0.4&29.2&19.6\\
\noalign{\smallskip} 
\hdashline
\noalign{\smallskip}  
\multicolumn{1}{l}{\textsc{\textbf{Continual Pre-training}}} \\
\noalign{\smallskip}
Balanced (400B ckpt.)&\texttt{+}100B&\texttt{+}100B&51.8&8.1&9.0&30.0&23.0\\
Code → Text &\texttt{+}180B&\texttt{+}20B&53.3&9.5&4.1&31.4&22.3\\
Balanced → Text&\texttt{+}180B&\texttt{+}20B&53.0&9.9&4.8&31.5&22.6\\
\noalign{\smallskip} 
\hdashline
\noalign{\smallskip} 
\multicolumn{1}{l}{\textsc{\textbf{Cooldown}}} \\
\noalign{\smallskip}
Text → Cooldown &\texttt{+}32B&\texttt{+}8B&54.4&11.4&4.4&32.9&23.4\\
Balanced → Cooldown &\texttt{+}32B&\texttt{+}8B&53.2&11.1&8.4&32.1&24.2\\
Code → Text → Cooldown &\texttt{+}32B&\texttt{+}8B&52.1&10.3&7.5&31.2&23.3\\
Balanced → Text → Cooldown &\texttt{+}32B&\texttt{+}8B&54.9&10.9&5.8&32.9&23.9\\
\bottomrule %% LOOKING GOOD!
\end{NiceTabular}
}
\caption{The Table above shows the different variants along with their average performance. }
%\yixuan{We could also consider using a Table to illustrate the token configurations of different variants}}
\label{tab:best-recipe}
\end{table*}
